Tackling Occlusion in Siamese Tracking with Structured Dropouts

Occlusion is one of the most difficult challenges in object tracking to model. This is because unlike other challenges, where data augmentation can be of help, occlusion is hard to simulate as the occluding object can be anything in any shape. In this paper, we propose a simple solution to simulate the effects of occlusion in the latent space. Specifically, we present structured dropout to mimick the change in latent codes under occlusion. We present three forms of dropout (channel dropout, segment dropout and slice dropout) with the various forms of occlusion in mind. To demonstrate its effectiveness, the dropouts are incorporated into two modern Siamese trackers (SiamFC and SiamRPN++). The outputs from multiple dropouts are combined using an encoder network to obtain the final prediction. Experiments on several tracking benchmarks show the benefits of structured dropouts, while due to their simplicity requiring only small changes to the existing tracker models.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> inference.tex <==

%\str{I am not sure if there is a need for such a long subsection. The idea described here is simple.
%You can apply the structured dropouts a. either at test time, on the computed feature maps of the new frames. Or b. you can also apply them at training time, thus having a model that is less sensitive to occlusions. In this case you could even not repeat the process in the new frame feature maps, as the model is trained against occlusion, thus saving some compute cycles. 
%
%Do we need to say more than these few lines? Do we really need a figure for this?
%}

%The results of multiple passes of structured dropouts are combined to infer the final prediction on the location of the target in the provided candidate image. We investigate two different approaches for this purpose: \emph{explicit} and \emph{implicit}. Schematic representations of the two inference processes for siamese trackers are shown in Figure \ref{ref_fig_schem_infer}. In explicit inference, dropouts are applied on the original pretrained models and the inference over all the results is performed as a post-processing step. Dropouts are applied only during the inference phase, and no additional model training is needed. In a conceptual sense, this approach can be interpreted similar to the way results for MC-Dropout are ensembled over a number of passes in \cite{Kraus2019arxiv}. In implicit inference, the process of inference is fused as a part of the model. Multiple cross-correlation activation maps, each obtained through a single dropout step, are combined to produce an activation map, which is then used to regress the bounding box location. This model needs to be trained end-to-end so as to teach the model to perform accurate inference. Details related to the two inference techniques for the proposed structured dropouts follow below. 

\begin{figure*}
\centering
\begin{subfigure}{1.0\textwidth}
\centering
\begin{tikzpicture}
\node (img) {\includegraphics[scale=0.45, trim= 0cm 8cm 3cm 0, clip]{images/concepts/fig_schem_exp.pdf}};
\node[] at (6.3,-0.4) {\small Prediction};
\node[] at (6.3,-0.8) {\small \{Cls, Loc\}};
\node[] at (4.2,-0.62) {\small Ensemble};
\node[] at (1.85,-0.5) {\small Pred-3};
\node[] at (1.85, 0.05) {\small Pred-2};
\node[] at (1.85, 0.6) {\small Pred-1};
\node[] at (1.85, -1.55) {\small Pred-$n$};
\node[] at (0.3,-0.5) {\small RPN};
\node[] at (0.3, 0.05) {\small RPN};
\node[] at (0.3, 0.6) {\small RPN};
\node[] at (0.3, -1.58) {\small RPN};
\node[] at (-4.2,-0.54) {\small SD-3};
\node[] at (-4.2, 0.05) {\small SD-2};
\node[] at (-4.2, 0.6) {\small SD-3};
\node[] at (-4.2, -1.58) {\small SD-$n$};
\node[] at (-8.0, 1.3) {Candidate};
\node[] at (-8.0, 0.9) {feature maps};
\node[] at (-8.0, 0.5) {$\Phi(x)$};
\node[] at (-8.0, -0.5) {Target};
\node[] at (-8.0, -0.9) {feature maps};
\node[] at (-8.0, -1.3) {$\Phi(z)$};
\node[] at (5.6, 1.35) { - cross-correlation};
\node[] at (5.63, 0.85) {RPN - Region proposal Net};
\node[] at (5.45, 0.38) {SD - Structured Dropout};
\end{tikzpicture}
\vspace{-2em}
\caption{Explicit}
\end{subfigure}
\begin{subfigure}{1.0\textwidth}
\vspace{-2em}
\centering
\begin{tikzpicture}
\node (img) {\includegraphics[scale=0.45, trim= 0cm 8cm 3cm 0, clip]{images/concepts/fig_schem_imp.pdf}};
\node[] at (6.2,-0.2) {\small Prediction};
\node[] at (6.2,-0.6) {\small \{Cls, Loc\}};
\node[] at (4.2,-0.33) {\small RPN};
\node[] at (2.45,-0.33) {\small Encode};
\node[] at (0.8, -0.33) {\small Stack};
\node[] at (-4.2,-0.54) {\small SD-3};
\node[] at (-4.2, 0.05) {\small SD-2};
\node[] at (-4.2, 0.6) {\small SD-3};
\node[] at (-4.2, -1.58) {\small SD-$n$};
\node[] at (-8.0, 1.3) {Candidate};
\node[] at (-8.0, 0.9) {feature maps};
\node[] at (-8.0, 0.5) {$\Phi(x)$};
\node[] at (-8.0, -0.5) {Target};
\node[] at (-8.0, -0.9) {feature maps};
\node[] at (-8.0, -1.3) {$\Phi(z)$};
\end{tikzpicture}
\vspace{-2em}
\caption{Implicit}
\end{subfigure}
\caption{Schematic representations of (a) explicit and (b) implicit inference methods for siamese tracking with structured dropouts.}
\label{ref_fig_schem_infer}
\end{figure*}

% \begin{figure*}
% \centering
% \begin{subfigure}{0.48\textwidth}
% \centering
% \includegraphics[height=3.5cm, width=8.7cm]{images/concepts/fig_schem_explicit.jpeg}
% \caption{Explicit Inference}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
% \centering
% \includegraphics[height=3.5cm, width=8.7cm]{images/concepts/fig_schem_implicit.jpeg}
% \caption{Implicit Inference}
% \end{subfigure}
% \caption{Full caption describing two inference processes goes here.}
% \label{ref_fig_schem_infer}
% \end{figure*}

% \begin{algorithm}[!t]
% \caption{Explicit Channel Dropout Sampling}
%     \begin{algorithmic}
%      \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%      \renewcommand{\algorithmicensure}{\textbf{Output:}}
%      \REQUIRE Prediction set $\mathcal{D}_t$
%      \ENSURE  Final box prediction $\overline{\mathbf{D}}_t$
%      \\ \textit{Initialisation} : $\mathcal{I} = \{\}$, $f = \{1, 1, ..., n$ times\};
%       \FOR {$j \in \{1, 2, ..., n\}$}
%           \IF {$j \in \mathcal{I}$}
%             \STATE continue
%           \ENDIF
%           \FOR {$k \in \{j+1, ..., n\}$}
%             \IF {$k \in \mathcal{I}$}
%                 \STATE continue
%             \ENDIF
%             \IF {$\text{IoU}(\mathbf{y}_{t,j}, \mathbf{y}_{t,k}) > \alpha_c$}
%                 \IF {$s_{t,j} > s_{t,k}$}
%                     \STATE $f_j = f_j+1$; add $k$ to $\mathcal{I}$;
%                 \ELSE
%                     \STATE $f_k = f_k+1$; add $j$ to $\mathcal{I}$;\\
% 				    continue;
%                 \ENDIF
%             \ENDIF
%           \ENDFOR
%       \ENDFOR \\
%  	$\overline{\mathbf{D}}_t = \mathbf{D}_{t,p}$, s.t. $p=\arg\max\limits_{i} f_i$ 
%     \end{algorithmic}
%     \label{algo_channel}
% \end{algorithm}

%\textbf{Explicit Inference.} For channel dropout, let $\gamma_i$ denote the fraction of channels of the feature map to be dropped at the $i^{\text{th}}$ inference step. Also, let the prediction by the tracking model at this step be denoted by $\mathbf{D}_{t,i} = \{\mathbf{y}_{t,i}, s_{t,i}\}$, where $\mathbf{y}_{t,i}$ and $s_{t,i}$ denote the predicted bounding box and the respective confidence score for the $i^{\text{th}}$ forward pass at time step $t$. From $n$ forward passes, the set of predictions can then be denoted as $\mathcal{D}_t = \{\mathbf{D}_{t,1}, \mathbf{D}_{t,2},\hdots, \mathbf{D}_{t,n}\}$. The final prediction $\overline{\mathbf{D}}_t$ is chosen from this set using the approach described in \mbox{Algorithm \ref{algo_channel}}. 

%In segment as well as slice dropouts, rather than dropping a few channels, a certain segment (all the channels depthwise) on the latent feature map is dropped at every pass, as shown in \mbox{Figure \ref{fig:dropout_ex1}}. In slice dropout, the number of passes $n$ are chosen to be a multiple of 4, denoted as $4k$. For $i \in \{1, 2, \hdots, k\}$, four passes are performed, each involving dropout of a slice starting from one of the four edges of the feature map. The value of $i$ defines the thickness of the slice.  For segment or slice dropout, let the area fraction of the dropout segment for the $i^{\text{th}}$ pass at step $t$ be denoted by $\mathcal{A}_{t,i}$. The confidence score for this box is then scaled up as $s^*_{t,i} = \frac{\mathcal{B}}{1-\mathcal{A}_{t,i}}\cdot s_{t,i}$. This is done to balance the drop in confidence score resulting from dropping out the patch. The constant $\mathcal{B}$ is added to control the impact of upscaling on the confidence scores. After upscaling, the bounding box with the highest value of $s^*_{t}$ is chosen as the final prediction for the current tracking step.

%\textbf{Implicit Inference.} In the implicit approach, the model is trained end-to-end to produce a single prediction, as demonstrated in Figure \ref{ref_fig_schem_infer}. Let $\tilde{\Phi}_{z,i}$ denote the modified feature map obtained after applying $i^{\text{th}}$ structured dropout on the template feature map $\Phi(z)$. Further, we denote the respective activation map obtained from cross-correlation with $\Phi(x)$ as $\Psi_{z_i,x}$. The concatenated activation set $\Psi_{z,x}$ is then constructed through concatenation of the activations from $n$ passes as $\Psi_{z,x} = [\Psi_{z_1,x}, \Psi_{z_2,x}, ..., \Psi_{z_n,x}]$. Further, $\Psi_{z,x}$ is passed through a set of convolutional layers, and the obtained output is then passed into the regression module (\emph{e.g.}, regional proposal network module in SiamRPN and SiamRPN++) similar to the conventional approach of Siamese tracking models. 

%Since implicit implementation involves additional convolutions applied on $\Psi_{z,x}$, the choice of these added convolutions depends on the type of dropouts. For example, slice dropouts are non-stochastic, and positional dependence of the each of the dropouts can be learned in the trained model. This implies that if trained on a diverse dataset with different scenarios of occlusions, the additional layers should learn the probabilities of occurrence of occlusion at the different edges of the target. With the series of convolutions, we expect the model to learn these positional values, be it that there are only limited cases of occlusion in our data. On the other hand, positional dependence cannot be learned for channel and segment dropouts due to their stochastic nature. However, the added convolutions are expected to learn operations applicable over a set. 

%The added encodings also depend on the choice of the base Siamese tracker. For example, SiamFC uses a cross-correlation layer to obtain a single channel response map for localizing the target. Thus, the added convolutions need to combine the $n$ feature maps in this case. For SiamRPN++, depthwise cross-correlation and layerwise aggregation produces 3 sets of activation maps, each containing $n \times N_c$ channels, where $N_c$ denotes the number of channels contained in the feature map before applying dropouts. Our choice of encodings for the two trackers are described in Section \ref{sec_imp_details}. 
